Time series modeling by a regression approach based on a latent process

Time series are used in many domains including finance, engineering, economics and bioinformatics generally to represent the change of a measurement over time. Modeling techniques may then be used to give a synthetic representation of such data. A new approach for time series modeling is proposed in this paper. It consists of a regression model incorporating a discrete hidden logistic process allowing for activating smoothly or abruptly different polynomial regression models. The model parameters are estimated by the maximum likelihood method performed by a dedicated Expectation Maximization (EM) algorithm. The M step of the EM algorithm uses a multi-class Iterative Reweighted Least-Squares (IRLS) algorithm to estimate the hidden process parameters. To evaluate the proposed approach, an experimental study on simulated data and real world data was performed using two alternative approaches: a heteroskedastic piecewise regression model using a global optimization algorithm based on dynamic programming, and a Hidden Markov Regression Model whose parameters are estimated by the Baum-Welch algorithm. Finally, in the context of the remote monitoring of components of the French railway infrastructure, and more particularly the switch mechanism, the proposed approach has been applied to modeling and classifying time series representing the condition measurements acquired during switch operations.

==> bibliographie_NN_2009_ <==
@BOOK{bishopPRML,
    Address        = {U K},
    Author         = {C. M. Bishop},
    Publisher      = {Springer Verlag},
    Title          = {Pattern recognition and machine learning},
    Year           = {2006},
}

@ARTICLE{dlr,
    Author         = {Dempster, A. P. and Laird, N. M.  and D. B. Rubin},
    Journal        = {Journal of The Royal Statistical Society, B},
    Pages          = {1-38},
    Title          = { Maximum likelihood from incomplete data via the EM algorithm},
    Volume         = {39(1)},
    Year           = {1977},
}

@ARTICLE{irls,
    Author         = {Green, P.},
    Journal        = {Journal of The Royal Statistical Society, B},
    Pages          = {149-192},
    Title          = {Iteratively Reweighted Least Squares for Maximum Likelihood Estimation, and some robust
and resistant alternatives},
    Volume         = {46(2)},
    Year           = {1984},
}

@ARTICLE{jordanHME,
    Author         = {Jordan, M. I. and Jacobs, R. A.},
    Journal        = {Neural Computation},
    Pages          = {181-214},
    Title          = {Hierarchical Mixtures of Experts and the EM algorithm},
    Volume         = {6},
    Year           = {1994},
    Language       = {\Eng}
}

@ARTICLE{chen99,
    Author         = {Chen, K. and L. Xu and Chi, H.},
    Journal        = {Neural Networks},
    Pages          = {1229-1252},
    Title          = {Improved learning algorithms for Mixture of Experts in multiclass classification},
    Volume         = {12(9)},
    Year           = {1999},
}

@ARTICLE{McGee,
    Author         = {McGee, V. E. and Carleton, W. T.},
    Journal        = {Journal of the American Statistical Association},
    Pages          = {1109-1124},
    Title          = {Piecewise regression},
    Volume         = {65},
    Year           = {1970},
}

@ARTICLE{sameSFC2007,
    Author         = {Samé, A. and Aknin, P. and Govaert, G.},
    Journal        = {Rencontres de la SFC, ENST, Paris},
    Pages          = {},
    Title          = {Classification automatique pour la segmentation des signaux unidimensionnels},
    Volume         = {},
    Year           = {2007},
}

@ARTICLE{jacobsME,
    Author         = {Jacobs, R. A. and Jordan, M. I. and Nowlan, S. J. and Hinton, G. E.},
    Journal        = {Neural Computation},
    Pages          = {79-87},
    Title          = {Adaptive Mixtures of Local Experts},
    Volume         = {1(3)},
    Year           = {1991},
}
%\bibitem{quandt} R. E. Quandt and and J. B. Ramsey, ``Estimating mixtures of normal distributions and switching regressions,"
%\emph{Journal of the American Statistical Association,} 73(364): 730752, 1978.

@ARTICLE{chen99,
    Author         = {Chen, K. and Xu, L. and Chi, H.},
    Journal        = {IEEE Transactions on Neural Networks},
    Pages          = {1229-1252},
    Title          = {Improved Learning Algorithms for Mixture of Experts in Multiclass Classification},
    Volume         = {9(12)},
    Year           = {1999},
}

@ARTICLE{rabiner,
    Author         = {Rabiner, L. R.},
    Journal        = {Proceedings of the IEEE},
    Pages          = {257-286},
    Title          = {A tutorial on hidden Markov models and selected applications in speech recognition},
    Volume         = {77(2)},
    Year           = {1989},
}

@ARTICLE{BaumWelch,
    Author         = {Baum, L.E., and Petrie, T., and Soules, G. and Weiss, N.},
    Journal        = {Annals of Mathematical Statistics},
    Pages          = {164-171},
    Title          = {A maximization technique occurring in the statistical analysis of probabilistic functions of Markov chains},
    Volume         = {41},
    Year           = {1970},
}

@TECHREPORT{fridman,
    Author         = {Fridman, M.},
    Institution    = {Institute of mathematics, University of Minnesota},
    Note           = {},
    Title          = {Hidden Markov Model Regression},
    Type           = {},
    Year           = {1993},
}

@ARTICLE{BIC,
    Author         = {Schwarz, G.},
    Journal        = {Annals of Statistics},
    Pages          = {461-464},
    Title          = {Estimating the dimension of a model},
    Volume         = {6},
    Year           = {1978},

@BOOK{reg_non_lin,
    Address        = {},
    Author         = {A. Antoniadis and J. Berruyer and R. Carmona},
    Publisher      = {Economica},
    Title          = {Régression non linéaire et applications},
    Year           = {1992},
}
%@BOOK{brei:frie:olsh:ston:1984,
%    Address        = {New York},
%    Author         = {Breiman, L. and J. H. Friedman and
%                      R. A. Olshen and C. J. Stone},
%    Publisher      = {Chapman and Hall},
%    Title          = {Classification And Regression Trees},
%    Year           = {1984},
%}

%@TECHREPORT{Daly:2003,
%    Author         = {Daly, Patrick W.},
%    Institution    = {CTAN (http://www.ctan.org/)},
%    Note           = {Describes the package natbib},
%    Title          = {Natural Sciences Citations and References (Author--Year and Numerical Schemes)},
%    Type           = {{\LaTeX} Package description},
%    Year           = {2003},
%}
%


